SN1987A neutrino burst: limits on flavor conversion

In this paper, we revisit the SN1987A neutrino data to see its constraints on flavor conversion. We are motivated by the fact that most works that analyze this data consider a specific conversion mechanism, such as the MSW (Mikheyev-Smirnov-Wolfenstein) effect, although flavor conversion is still an open question in supernovae due to the presence of neutrino-neutrino interactions. In our analysis, instead of considering a specific conversion mechanism, we let the electron antineutrino survival probability $P_{\overline{e}\overline{e}}$ be a free parameter. We fit the data from Kamiokande-II, Baksan, and IMB detected spectrum with two classes of models: time-integrated and time-dependent. For the time-integrated model, it is not possible to put limits above $1\sigma$ (68% confidence level) on the survival probability. The same happens for the time-dependent model when cooling is the only mechanism of antineutrino emission. However, for models considering an accretion phase, $P_{\overline{e}\overline{e}}\sim0$ is strongly rejected, showing a preference for the existence of an accretion component in the detected antineutrino flux, and a preference for normal mass ordering when only the MSW is present.

==> Apendices/Likelihood.tex <==
\subsection{Marcos}
The likelihood can be derived using a Poissonian p.d.f.  $P_i(x_i,\textbf{y})$, where $x_i$ and $\textbf{y}$ accounts measured variables (e.g. $x_i = t_i, E_i, \theta_i$ or combination of them in each bin $i$) and parameters from a model respectively, then

\begin{equation}
    \mathcal{L} = \prod^{N_{bins}}_{i=1} P_i(x_i, \textbf{y})
\end{equation}

\begin{equation}\label{eq:poissonian likelihood}
    \mathcal{L} = \prod_{i=1}^{N_{bins}} \frac{{\mu(x_i, \textbf{y})}^{n_i}}{n_i!} e^{-\mu(x_i, \textbf{y})}.
\end{equation}
The mean of the distribution can be interpreted as the number of events in a bin size of $\delta x_i$, thus $\mu(x_i, \textbf{y}) = \delta x_i R(x_i, \textbf{y})$, and the likelihood becomes

\begin{equation}\label{eq:poissonian likelihood}
    \mathcal{L} = e^{-\sum_i^{N_{bins}} \delta x_i R(x_i, \textbf{y})} \prod_{i=1}^{N_{bins}} \frac{{[\delta x_i R(x_i, \textbf{y})]}^{n_i}}{n_i!} .
\end{equation}
As in the SN1987A we have low statistics, a binned likelihood could lead a loss of information, once any choice of event distribution on the bin would be arbitrary. To go around this, it is possible to make an infinitesimal size of bin $\delta x_i \rightarrow dx_i$, making the sum in the exponential becomes an integral. In this scenario, the bins have 1 or 0 events, then considering only the ones with events, dropping the others and making $n_i \rightarrow 1$, changes the likelihood to

\begin{equation}\label{eq:poissonian likelihood}
    \mathcal{L} = e^{-\int dx R(x, \textbf{y})} \prod_{i=1}^{N_{obs}} dx_i R(x_i, \textbf{y}),
\end{equation}
with $N_{obs}$ being the number of observed events, for a unbinned likelihood, where in our analysis $dx = dtdEd\cos\theta$. Details in the inclusion of background, efficiency and other additions (not exactly directly adopted by us) to the likelihood can be seen in \cite{ianni2009likelihood} and \cite{jegerlehner1996neutrino}.


\subsection{Dedin}

\added[id=Dedin]{Here we describe another way to derive the extended likelihood expression used in this work. In addition to the usual likelihood, where we multiply the probability density $f(x_i,\textbf{y})$ of a given of a set of $N$ measurements $x_i$  with model parameters $\textbf{y}$, the extended likelihood multiply the usual one by the probability of getting N number of events, considering that it follows a Poisson distribution with an expected number of events $\nu$. Therefore, we can define it as follows.

\begin{equation}
    \mathcal{L}_{ext}(\mathbf{\textbf{y}})= \frac{\nu^n}{N!} e^{-\nu} \prod_{i=1}^N f(x_i,\mathbf{\textbf{y}}) = \frac{e^{-\nu}}{N!} \prod_{i=1}^N \nu f(x_i,\mathbf{\textbf{y}}) 
\end{equation}

This method finds the set of parameters $\hat{\textbf{y}}$ that best-fit the data by maximizing the likelihood. We can improve this method by considering that the event may come from the signal (supernova) or a background source. In this case we can consider that the expected number of events $\nu$ have a signal contribution corresponding to a fraction $f_s$, and a contribution from the background, corresponding to a fraction $(1-f_s)$, so that $\nu=\nu_s+\nu_b = f_s\nu+(1-f_s)\nu$. Therefore, we can rewrite the likelihood as

\begin{equation}
\begin{split}
     \mathcal{L}_{ext}(\mathbf{\textbf{y}})=& \frac{e^{-(\nu_s+\nu_b)}}{N!} \prod_{i=1}^N \nu [f_sp_s(x_i,\textbf{y})+(1-f_s)p_b(x_i,\textbf{y})]\\ =& \frac{e^{-(\nu_s+\nu_b)}}{N!} \prod_{i=1}^N [\nu_sp_s(x_i,\textbf{y})+\nu_b p_b(x_i,\textbf{y})]    
\end{split}
\end{equation}

Where $p_s(x_i,\textbf{y})$ and $p_b(x_i,\textbf{y})$ are the p.d.f. for the signal and background respectively. In our case,  $\nu_s p_s(x_i,\textbf{y})$ and $\nu_b p_b(x_i,\textbf{y})$ correspond to the event rate $R(x,\textbf{y})$ and the background rate $B=B(E_i)$ respectively. In this case, the measured variables are the positron measured energy, time and cosine $x_i={E_{e,i},t_i,\cos{\theta_i}}$ and the parameters $\textbf{y}$ are the ones related to the astronomical emission models and to the flavor conversion mechanism. 

In our treatment, as in \cite{Pagliaroli:2008ur}, we consider that the time and angle uncertainties are irrelevant \footnote{colocar um exemplo das incertezas?}. However, the energy uncertainties are relevant and we introduce it by integrating over all possible measured energies considering a multiplication (conditional) by a Gaussian $\mathcal{L}_i(E_e)$ with mean in the measured energy $E_e$ and width corresponding to the uncertainty $\delta E_e$.

\begin{equation}
    \mathcal{L}_{ext}(\mathbf{\textbf{y}})\approx e^{-f_d \int R(t) dt}\prod_{i=1}^N e^{R(t_i)\tau_d} \left[\frac{B_i}{2}+\int R(t_i,E_{e,i},\cos\theta_i)\mathcal{L}_i(E_e) dE_e \right]
\end{equation}

Here, we have considered that the total number of background events is irrelevant when compared to the total number of signal events $\nu_s>>\nu_b$, eliminating it in the exponential. However, the probability of one event being from the background is relevant, so it remains in our event rate contribution. Also, we consider the deadtime of each event $\tau_d$ for each detector ($d=K,B,I$), so that $\nu_s = f_d \int R(t) dt - \sum_{i=1}^N R(t_i) \tau_d$. In the case of the time-independent model, we only have to consider a time integration in the event rate for the signal $R(t_i,E_{e,i},\cos\theta_i)$ and for the background $B(E_i)$).}

